Why Do Developers Get Password Storage Wrong? A Qualitative Usability Study

Passwords are still a mainstay of various security systems, as well as the cause of many usability issues. For end-users, many of these issues have been studied extensively, highlighting problems and informing design decisions for better policies and motivating research into alternatives. However, end-users are not the only ones who have usability problems with passwords! Developers who are tasked with writing the code by which passwords are stored must do so securely. Yet history has shown that this complex task often fails due to human error with catastrophic results. While an end-user who selects a bad password can have dire consequences, the consequences of a developer who forgets to hash and salt a password database can lead to far larger problems. In this paper we present a first qualitative usability study with 20 computer science students to discover how developers deal with password storage and to inform research into aiding developers in the creation of secure password systems.

==> tableExpertise.tex <==
\begin{table}[tb]
\footnotesize
\centering
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{ c P{6cm} P{6.5cm} }
\toprule
    & Questions & Rating Scale \\ \midrule
    Q1 & I have a good understanding of security concepts. & Strongly disagree (1) - Strongly agree (7)\\ \midrule
    Q2 & How often do you ask for help facing security problems? & Never (1) - Every time (7)\\ \midrule
    Q3 & How often are you asked for help when somebody is facing security problems? & Never (1) - Every time (7)\\ \midrule
    Q4 & How often do you need to add security to the software you develop in general (Primed Group: apart from this study)? & Never (1) - Every time (7)\\ \midrule
    Q5 & How often have you stored passwords in the software you have developed (Primed Group: apart from this study)? & Never (1) - Every time (7)\\ \midrule
    Q6 & How would you rate your background/knowledge with regard to secure password storage in a database? & Not knowledgeable at all (1) - Very knowledgeable (7) \\ 
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Participants' Security Expertise and Background Knowledge about Password Storage}
\label{table:securityExpertiseQuestions}
\end{table}

==> table_implemented_solutions.tex <==
\begin{table}[tb]
\footnotesize
\centering
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{c  c  c }
\toprule
    & \textbf{Hash Function} & \textbf{Salt}
    \\ \midrule
    P1 & BCrypt & \texttt{SecureRandom} \\
    P2 & PBKDF2WithHmacSHA1& \texttt{SecureRandom} \\
    P3 & BCrypt & \texttt{SecureRandom}\\
    P4 & PBKDF2WithHmacSHA512 & \texttt{SecureRandom}\\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Password Storage Implementations}
\label{table:implementedSolutions}
\end{table}
